A machine learning-based selective sampling procedure for identifying the low energy region in a potential energy surface: a case study on proton conduction in oxides

In this paper, we propose a selective sampling procedure to preferentially evaluate a potential energy surface (PES) in a part of the configuration space governing a physical property of interest. The proposed sampling procedure is based on a machine learning method called the Gaussian process (GP), which is used to construct a statistical model of the PES for identifying the region of interest in the configuration space. We demonstrate the efficacy of the proposed procedure for atomic diffusion and ionic conduction, specifically the proton conduction in a well-studied proton-conducting oxide, barium zirconate BaZrO3. The results of the demonstration study indicate that our procedure can efficiently identify the low-energy region characterizing the proton conduction in the host crystal lattice, and that the descriptors used for the statistical PES model have a great influence on the performance.

==> figtab.tex <==
% ***************************************************************************
% sec II
% ***************************************************************************

%\clearpage
% ---------------------------------------------------------------------------
% Fig01 GPSampling-Example
% ---------------------------------------------------------------------------
\begin{figure*}[p]
 \begin{center}
  \begin{tabular}{ccc}
   \multicolumn{3}{c}{\includegraphics[width=0.75\textwidth]{Fig/Fig01-GPSampling-Example/key.eps}} \\
   \includegraphics[width=0.33\textwidth]{Fig/Fig01-GPSampling-Example/lowPERegion/plot_ai.eps} &
   \includegraphics[width=0.33\textwidth]{Fig/Fig01-GPSampling-Example/step0/plot.eps} &
   \includegraphics[width=0.33\textwidth]{Fig/Fig01-GPSampling-Example/step1/plot.eps} \\
   (a) low PE region &
   (b) step0 (initialization) &
   (c) step1 \\
   \includegraphics[width=0.33\textwidth]{Fig/Fig01-GPSampling-Example/step2/plot.eps} &
   \includegraphics[width=0.33\textwidth]{Fig/Fig01-GPSampling-Example/step3/plot.eps} &
   \includegraphics[width=0.33\textwidth]{Fig/Fig01-GPSampling-Example/step4/plot.eps} \\
   (d) step2 &
   (e) step3 &
   (f) step4 \\	   
   \includegraphics[width=0.33\textwidth]{Fig/Fig01-GPSampling-Example/step5/plot.eps} &
   \includegraphics[width=0.33\textwidth]{Fig/Fig01-GPSampling-Example/step6/plot.eps} &
   \includegraphics[width=0.33\textwidth]{Fig/Fig01-GPSampling-Example/step7/plot.eps} \\
   (g) step5 &
   (h) step6 &
   (i) step7 \\	   
   \includegraphics[width=0.33\textwidth]{Fig/Fig01-GPSampling-Example/step8/plot.eps} &
   \includegraphics[width=0.33\textwidth]{Fig/Fig01-GPSampling-Example/step9/plot.eps} &
   \includegraphics[width=0.33\textwidth]{Fig/Fig01-GPSampling-Example/step10/plot.eps} \\
   (j) step8 &
   (k) step9 &
   (l) step10 \\	   
   \includegraphics[width=0.33\textwidth]{Fig/Fig01-GPSampling-Example/step11/plot.eps} &
   \includegraphics[width=0.33\textwidth]{Fig/Fig01-GPSampling-Example/step12/plot.eps} &
   \includegraphics[width=0.33\textwidth]{Fig/Fig01-GPSampling-Example/step13/plot.eps} \\
   (m) step11 &
   (n) step12 &
   (o) step13 \\	   
   \includegraphics[width=0.33\textwidth]{Fig/Fig01-GPSampling-Example/step14/plot.eps} &
   \includegraphics[width=0.33\textwidth]{Fig/Fig01-GPSampling-Example/step15/plot.eps} &
   \includegraphics[width=0.33\textwidth]{Fig/Fig01-GPSampling-Example/step16/plot.eps} \\
   (p) step14 &
   (q) step15 &
   (r) step16 \\	   
  \end{tabular}
  \caption{
  Schematic illustration of the proposed selective sampling procedure 
  in one-dimensional configuration space with synthetic data. 
  %
  In each plot, 
  the X and Y-axes represent 
  the configuration space and the PEs, respectively.
%
The PES and its $N=50$ points are shown as a 
black solid curve
and 
squares, respectively.
%
In plot (a), 
the low PE region with $\alpha = 0.20$ is represented by a blue bar.
%
The goal in this example is to efficiently identify and evaluate the PEs at the 9 points within this blue bar region. 
%
Plot (b) indicates the initialization step,
where two points (filled squares) are randomly selected and their PEs are evaluated.
%
The remaining 16 plots (plots (c) to plot (r))
indicate steps 1 to 16 of the procedure. 
%
At each step,
a point is selected and the PE is evaluated
by using the GP-based statistical model,
where
the points selected so far are shown as filled squares. 
%
In each plot, 
the predicted PEs and their uncertainties
given by the GP-based statistical model are depicted by 
a red solid curve and shaded region,
respectively. 
%
In addition,
the true and the estimated threshold values
$\theta_\alpha$
and 
$\hat{\theta}_\alpha$
are shown as black and red broken lines,
respectively. 
%
In this example, 
the 9 points in the low PE region are successfully identified
and the threshold is also correctly estimated
at step 16 (plot (r)).
  }
  \label{fig:GPSampling-Example}
 \end{center}
\end{figure*}

% ***************************************************************************
% sec III
% ***************************************************************************

%\clearpage
% ---------------------------------------------------------------------------
% Fig02 BaZrO3
% ---------------------------------------------------------------------------
\begin{figure*}[p]
\begin{center}
\includegraphics[width=.22\textwidth]{Fig/Fig02-BaZrO3/plot_a} 
\includegraphics[width=.185\textwidth]{Fig/Fig02-BaZrO3/plot_b} 
\caption{
(a) Crystal structure of ${\rm BaZrO_3}$. 
(b) Asymmetric unit in the unit cell of ${\rm BaZrO_3}$.
}
\label{fig:BaZrO3}
\end{center}  
\end{figure*}

%\clearpage
% ---------------------------------------------------------------------------
% Fig03 PE-relaxed
% ---------------------------------------------------------------------------
\begin{figure*}[p]
\begin{center}
\includegraphics[width=.42\textwidth]{Fig/Fig03-PE-Relaxed/plot}
\caption{PES of a proton in the low PE region ($\alpha = 0.2$) obtained by DFT calculations with structural optimization for ${\rm BaZrO_3}$. 
The low PE region ($\alpha = 0.2$) at which the PEs are lower than 0.30 eV is surrounded by yellow surfaces. }
\label{fig:PE-relaxed}
\end{center}  
\end{figure*}

% ***************************************************************************
% sec IV
% ***************************************************************************

%\clearpage
% ---------------------------------------------------------------------------
% Fig04 Result-Efficiency
% ---------------------------------------------------------------------------
\begin{figure*}[p]
\begin{center}
\includegraphics[width=0.75\textwidth]{Fig/Fig04-Result-Efficiency/plot1.eps} \\
(a) $\alpha=0.05$ \\
\includegraphics[width=0.75\textwidth]{Fig/Fig04-Result-Efficiency/plot2.eps} \\
(b) $\alpha=0.10$ \\
\includegraphics[width=0.75\textwidth]{Fig/Fig04-Result-Efficiency/plot3.eps} \\
(c) $\alpha=0.20$ \\
\caption{
 Efficiencies of the seven sampling methods for
 (a) $\alpha = 0.05$,
 (b) $\alpha = 0.10$ and
 (c) $\alpha = 0.20$. 
 %
 The numbers of grid points
 successfully sampled from the low PE region 
 (\#(TP))
 are plotted
 as functions of 
 the number of PE evaluations by DFT computations 
 (\#(TP) + \#(FP)). 
}
\label{fig:result-efficiency}
\end{center}
\end{figure*}

% ---------------------------------------------------------------------------
% Fig05 sampling-points
% ---------------------------------------------------------------------------
%\clearpage
\begin{figure*}[p]
 \begin{center}
  \begin{tabular}{cccc}
   100 steps & 200 steps & 300 steps & 400 steps \\
   \hline
\multicolumn{4}{c}{{\tt GP1} sampling} \\ \hline
\includegraphics[width=.175\textwidth]{Fig/Fig05-sampling-points/plot_GPwithoutApproxPES100.eps} &
\includegraphics[width=.175\textwidth]{Fig/Fig05-sampling-points/plot_GPwithoutApproxPES200.eps} &
\includegraphics[width=.175\textwidth]{Fig/Fig05-sampling-points/plot_GPwithoutApproxPES300.eps} &
\includegraphics[width=.175\textwidth]{Fig/Fig05-sampling-points/plot_GPwithoutApproxPES400.eps} \\
\hline
\multicolumn{4}{c}{{\tt GP4}  sampling} \\ \hline
\includegraphics[width=.175\textwidth]{Fig/Fig05-sampling-points/plot_GPwithApproxPES100.eps} &
\includegraphics[width=.175\textwidth]{Fig/Fig05-sampling-points/plot_GPwithApproxPES200.eps} &
\includegraphics[width=.175\textwidth]{Fig/Fig05-sampling-points/plot_GPwithApproxPES300.eps} &
\includegraphics[width=.175\textwidth]{Fig/Fig05-sampling-points/plot_GPwithApproxPES400.eps} \\
\hline
\multicolumn{4}{c}{{\tt prePES} sampling} \\ \hline
\includegraphics[width=.175\textwidth]{Fig/Fig05-sampling-points/plot_naive100.eps} &
\includegraphics[width=.175\textwidth]{Fig/Fig05-sampling-points/plot_naive200.eps} &
\includegraphics[width=.175\textwidth]{Fig/Fig05-sampling-points/plot_naive300.eps} &
\includegraphics[width=.175\textwidth]{Fig/Fig05-sampling-points/plot_naive400.eps} \\
\hline
\multicolumn{4}{c}{{\tt random} sampling} \\ \hline
\includegraphics[width=.175\textwidth]{Fig/Fig05-sampling-points/plot_random100.eps} &
\includegraphics[width=.175\textwidth]{Fig/Fig05-sampling-points/plot_random200.eps} &
\includegraphics[width=.175\textwidth]{Fig/Fig05-sampling-points/plot_random300.eps} &
\includegraphics[width=.175\textwidth]{Fig/Fig05-sampling-points/plot_random400.eps} \\
\hline
\multicolumn{4}{c}{{\tt ideal} sampling} \\ \hline
\includegraphics[width=.175\textwidth]{Fig/Fig05-sampling-points/plot_ideal100.eps} &
\includegraphics[width=.175\textwidth]{Fig/Fig05-sampling-points/plot_ideal200.eps} &
\includegraphics[width=.175\textwidth]{Fig/Fig05-sampling-points/plot_ideal300.eps} &
\includegraphics[width=.175\textwidth]{Fig/Fig05-sampling-points/plot_ideal353.eps} \\
\end{tabular}
\caption{
  Selected grid points
  (gray dots)
  at 100, 200, 300, and 400 steps
  by different sampling methods
  in the model crystal lattice of ${\rm BaZrO_3}$
  for $\alpha = 0.20$ case.
  %
  The yellow surface
  in each plot is the isosurface
  corresponding to the energy threshold at $\alpha = 0.2$.
  }
  \label{fig:sampling-points}
 \end{center}
\end{figure*}

%% ---------------------------------------------------------------------------
%% OBS PE-fixed
%% ---------------------------------------------------------------------------
%\begin{figure*}[p]
%\begin{center}
%\includegraphics[width=.42\textwidth]{Fig/Fig06-PE-Fixed/plot}
%\caption{A preliminary PES of a proton obtained by single point DFT computations with fixed lattice  in the model host crystal  ${\rm BaZrO_3}$. The low PE region at which the PEs are lower than 1.6 eV  (roughly corresponding to the lower 20\% value of the preliminary PEs of all the $N = 1768$ grid points) is surrounded by yellow surfaces.}
%\label{fig:PE-fixed}
%\end{center}  
%\end{figure*}

% ---------------------------------------------------------------------------
% Fig06 Rank-Correlation
% ---------------------------------------------------------------------------
%\clearpage
\begin{figure*}[p]
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=.35\textwidth]{Fig/Fig06-Rank-Correlation/plot1} &
\includegraphics[width=.35\textwidth]{Fig/Fig06-Rank-Correlation/plot2} \\
(a) {\tt prePES} &
(b) {\tt GP4} \\
\end{tabular}
\caption{Rank correlation between the actual and the preliminary PEs. 
The grid points in $\cP_\alpha$ are shown as open circles, while those in $\cN_\alpha$ are shown as crosses. 
Sampled points at 400 steps are also shown as blue and red symbols in
 (a) {\tt prePES} and (b) {\tt GP4}, respectively, for the $\alpha = 0.20$ case. 
The method {\tt GP4} samples all the positive points at 400 steps with a small number of false positives, i.e., sampled points that are not included in the low PE region.
Therefore, in (b), there are no false negative points. 
}
\label{fig:rank-correlation}
\end{center}
\end{figure*}

% ---------------------------------------------------------------------------
% Fig07 Want-Find
% ---------------------------------------------------------------------------
%\clearpage
\begin{figure*}[p]
 \begin{center}
  \begin{tabular}{cc}
   %\includegraphics[width=.4\textwidth]{Fig/Fig07-Want-Find/wantFind.eps} &
   %\includegraphics[width=.4\textwidth]{Fig/Fig07-Want-Find/notFound.eps} \\
   (a) Grid points in the low PE region with $\alpha = 0.2$ &
   (b) Grid points that could not be found by {\tt prePES}
  \end{tabular}
  \caption{
  (a) Grid points
  in the low PE region
  with
  $\alpha = 0.2$
  of
  ${\rm BaZrO_3}$, 
  and
  (b)
  grid points
  that could not be found
  via the {\tt prePES} sampling method 
  in 394 steps
  by which
  the {\tt GP4} sampling method could successfully identify all the grid points in the low PE region. 
  %
  Plot (b) indicates that 
  grid points around the O atom (red) could not be correctly identified
  by using preliminary PES alone,
  i.e., 
  the preliminary PEs
  at these points are NOT relatively low, 
  although
  their actual PEs are found to be relatively low 
  after structural optimization. 
  }
  \label{fig:points-not-found}
 \end{center}
\end{figure*}

% ---------------------------------------------------------------------------
% Tab01 Result-Efficiency
% ---------------------------------------------------------------------------

%\clearpage
\begin{table}[t]
 \caption{
 Numbers of sampling steps
 required to identify all the grid points in the low PE region. 
 %
 The averages and the standard deviations
 over 10 runs
 with different random seeds
 are shown.
 %
 Note that
 the results of {\tt prePES} are obtained
 by a single run
 because there is no random component in {\tt prePES}.}
 \label{tab:result-efficiency}
 \begin{center}
  \begin{tabular}{c||c|c|c}
   & $\alpha=0.05$ & $\alpha=0.10$ & $\alpha=0.20$ \\ \hline
   {\tt GP1}& 
   $1488.5 \pm 239.4$ & 
   $1576.1 \pm 36.9$ & 
   $1539.6 \pm 31.2$ 
   \\
   {\tt GP2}& 
   $1294.1 \pm 180.9$ & 
   $1266.9 \pm 167.9$ & 
   $1269.4 \pm 100.3$ 
   \\
   {\tt GP3}& 
   $511.7 \pm 30.4$ & 
   $617.6 \pm 49.7$ & 
   $875.2 \pm 60.1$ 
   \\
   {\tt GP4} & 
   $114.3 \pm 1.3$ &
   $235.5 \pm 1.0$ &
   $394.1 \pm 5.2$
   \\
   {\tt random} & 
   $1749.6 \pm 15.0$ & 
   $1757.1 \pm 11.3$ & 
   $1762.2 \pm 3.9$ 
   \\
   {\tt prePES} & 
   $592$ & 
   $1222$ & 
   $1479$ 
   \\ \hline
   {\tt ideal}  &
   $89$ &
   $177$ &
   $354$ \\	       
  \end{tabular}
 \end{center}
\end{table}

% ***************************************************************************
% sec V
% ***************************************************************************

% ---------------------------------------------------------------------------
% Fig08 stopping-criterion
% ---------------------------------------------------------------------------
%\clearpage
\begin{figure*}[p]
 \begin{center}
   \includegraphics[width=.50\textwidth]{Fig/Fig08-stopping-condition/plot1.eps} \\
   (a) The estimated FNR \\
   \includegraphics[width=.50\textwidth]{Fig/Fig08-stopping-condition/plot2.eps} \\
   (b) The estimated threshold \\
   \caption{The profiles of the estimated FNRs and thresholds for $\alpha = 0.20$ case.}
   \label{fig:stopping-condition}
 \end{center}
\end{figure*}

% ---------------------------------------------------------------------------
% Fig09 stopping-criterion
% ---------------------------------------------------------------------------
%\clearpage
\begin{figure*}[p]
 \begin{center}
   \includegraphics[width=.50\textwidth]{Fig/Fig09-select-alpha/plot1.eps} \\
   (a) Sampling profile  \\
   \includegraphics[width=.50\textwidth]{Fig/Fig09-select-alpha/plot2.eps} \\
   (b) FNR \\
   \includegraphics[width=.50\textwidth]{Fig/Fig09-select-alpha/plot3.eps} \\
   (c) Threshold \\
   \caption{Results when $\alpha$ is gradually increased as 0.05 $\to$ 0.10 $\to$ 0.15 $\to$ 0.20 in a stepwise manner. (a) THe true positive points, (b) the estimated FNR, and (c) the estimated threshold are plotted as functions of the numbers of DFT computations. Here, $\alpha$ is updated when the estimated false negative rate $\hat{\rm FNR}$ becomes less than $\veps = 10^{-6}$ at the current $\alpha$. Note that the FNR in (b) and the threshold in (c) change with $\alpha$.}
   \label{fig:select-alpha} \end{center}
\end{figure*} 
